Intention as Commitment toward Time

In this paper we address the interplay among intention, time, and belief in dynamic environments. The first contribution is a logic for reasoning about intention, time and belief, in which assumptions of intentions are represented by preconditions of intended actions. Intentions and beliefs are coherent as long as these assumptions are not violated, i.e. as long as intended actions can be performed such that their preconditions hold as well. The second contribution is the formalization of what-if scenarios: what happens with intentions and beliefs if a new (possibly conflicting) intention is adopted, or a new fact is learned? An agent is committed to its intended actions as long as its belief-intention database is coherent. We conceptualize intention as commitment toward time and we develop AGM-based postulates for the iterated revision of belief-intention databases, and we prove a Katsuno-Mendelzon-style representation theorem.

==> sections/coherence-condition-proof.tex <==
\section{Coherence Condition Proofs}

\setcounter{lemma}{0}

\begin{lemma}
\label{lemma:cohere_subset}
if $I'\subseteq I$, then $Cohere(I)\vdash Cohere(I')$.
\end{lemma}

\begin{proof}
Suppose an intention database $I=\{(a_{t_1},t_1),\ldots,(a_{t_n},t_n)\}$ with $t_1<\ldots<t_n$. Recall that
\begin{flalign*}
Cohere(I) = \Diamond_0\bigvee_{\substack{a_k\in Act{} : k\not\in\{t_1,\ldots, t_n\}\\a_k=b_k : k\in\{t_1,\ldots,t_n\}}} pre(a_{t_1},a_{t_{1}+1},\ldots,a_{t_n})_{t_1}.
\end{flalign*}
Suppose $I'\subset I$, so we have
\begin{flalign*}
Cohere(I') = \Diamond_0\bigvee_{\substack{a_k\in Act{} : k\not\in\{t_1,\ldots, t_n\}\\a_k=b_k : k\in\{t_1,\ldots,t_n\}}} pre(a_{t_1},a_{t_{1}+1},\ldots,a_{t_n})_{t_1}.
\end{flalign*}
\end{proof}

==> sections/introduction-old.tex <==
\section{Introduction}

Sometime in the near future you will tell your household robot: ``Bobby, get me some beer from the store''. Bobby confirms your request, but when its walking to the store it encounters your partner, who says: ``Bobby, our house is a mess, go home and clean''. Bobby returns home, takes the mop out of its closet and prepares to start cleaning. Just as it is ready to make its first swipe, one of your friends walks in asking: ``Bobby, it has been snowing outside, could you clean my car?''. In the meantime, you are getting increasingly frustrated by your lack of beer, and when you see Bobby in the kitchen you shout: ``You still didn't get my beers? Go get them immediately!''. After letting Bobby run around for a few days you return the robot to the factory complaining it does not finish any of the tasks it starts with.

When Bobby 2.0 arrives, the manufacturer happily tells you the new settings will no longer cause Bobby to drop its commitments so quickly. Delighted, you exclaim: ``Bobby, I have some friends coming over tonight, get some ingredients and cook diner so we can eat at 7pm tonight''. Realizing the shop closes only at 5pm, Bobby 2.0 delays going to the grocery story until the very last moment, hereby keeping its schedule free for other possible tasks. Unexpectedly, on its way to the grocery store Bobby is delayed by an open bridge and arrives at the store minutes after closing time. It returns to your home empty-handed, leaving you and your friends hungry. It turns out Bobby 2.0 is delaying every until just before the deadline. Since tasks often have unexpected delays, this means that most of the tasks are finished too late, or not at all. Frustrated, you return it to the factory again, complaining that Bobby is procrastinating its commitments.

On return, the manufacturer ensures you that Bobby 3.0 will no longer postpone fulfilling its commitments, nor will it drop them quickly. At this time you are rather skeptical, but still you ask: ``Bobby, I'd like to have diner tonight again. Please buy the ingredients at 2pm, and cook for me at 6pm''. Around 12pm, your partner again realizes the house hasn't been cleaned properly for a long time, and therefore tells Bobby to clean the house intensively. At 6pm, you sit at your kitchen table wondering where diner is, so you call Bobby asking what happened. Bobby explains it had to clean the house at 12pm, which took three hours, so it couldn't fulfill its commitment to go shopping at 2pm.

Disappointed, you return it to the manufacturer where it is dismantled.

\subsection{Commitment to Time}

The example above is very similar to the example of Willie the robot, due to~\cite{Cohen1990}. In their article entitled ``Intention = Choice + Commitment'', Cohen and Levesque were interested in specifying the rational balance of autonomous agents, focusing on the role that intention plays in maintaining this balance. Their approach has typified much subsequent research on belief-desire-intention (BDI) logics, namely to understand and study intentions as commitment in relation to goals and desires. For instance,~\cite{Rao1991} define various commitment strategies of an agents, from blindly committed towards goals, to open mindedly committed. A popular approach is to specify a temporal logic such as linear-time logic (LTL) or computational-tree logic (CTL*) and use modal operators for mental states and use expression of the form ``some time in the future'', or ''in the next time moment'' to reason about the temporal behavior.

In approaches following the ideas of Cohen and Levesque~\citep{Rao1991, Meyer1999} are two examples), intention is often defined as commitments towards goals . However, being committed towards a goal is only one dimension of a commitment, while they have many more aspects. One important aspect of a commitment that we focus on in this article is \emph{commitment towards time}, i.e., \emph{when} these commitments will be fulfilled. In the example above, Bobby the robot is an \emph{online system}; it is receiving orders, forming plans, scheduling tasks, and executing them, all in parallel and in real-time. Bobby plans its commitments at appropriate moments, making sure the different plans do not overlap or are incompatible, while it at the same time may receive new instructions from users. 

When specifying a system \emph{exogenously}, which has typified much work on philosophical logic, it may be sufficient to reason about behaviors with notions such as ``Bobby believes it should do shopping some time in the future'', or ``in the next time moment, Bobby intends to make diner''. However, if we specify a system \emph{endogenously}, which typifies much work in computer science and planning, one has to be more precise about when commitments will be fulfilled. Indeed, Bobby should know it has the commitment to go shopping at 2pm, and not some time in the future, so that its planner can continue planning on this assumption. By focusing on commitments towards time we therefore aim to bridge the gap between logics of agency on the one side and computer science and planning on the other side. 

We will see that even in a simplified setting where we only consider commitments towards time, already non-trivial complications arise. Commitments play the role of \emph{assumptions} on which further plans are based. The three versions of Bobby the household robot each use a different behavior when it comes to commitment to time. The first version uses a stack-like data structure in order to execute its tasks: it adds each new commitments on the stack, and then executes the tasks on top of its stack. The second version rather uses a queue, and moreover delays executing these tasks until the very last moment. Finally, the last version is able to schedule its commitments in time, but it cannot reschedule them. None of these versions seem to be able to fulfilled commitments in a desired way. Instead, Bobby should be able to make plans, store the commitments and use these as assumptions in further planning.

Commitment towards time plays an even bigger role in a multi-agent setting. \todo{Elaborate on coordination}



\subsection{Methodology}

\begin{figure}[ht]
\centering
\includegraphics[scale=0.33]{img/dbperspective}
\caption{The database perspective}
\label{fig:dbperspective}
\end{figure}

We view the problem of intention revision as a database management problem (see~\citep{Shoham2009} for more on the conceptual underpinnings of this standpoint). At any given moment, an agent must keep track of a number of facts about the current situation. This includes beliefs about the current state, beliefs about possible future states, which actions are available now and in the future, and also what the agent plans to do at future moments. It is important that all of this information be jointly consistent at any given moment and furthermore can be modified as needed while maintaining consistency.

In this article we introduce a simple logic that formally models such a ``database''. That is, \emph{consistency} in this logic is meant to represent not only that the agent's beliefs are consistent and the agent's future plan is consistent, but also that the agent's beliefs and intentions together form a \emph{coherent} picture of what may happen, and of how the agent's own actions will play a role in what happens. Our primary contribution in this article is to focus also on how the database is to be modified, and in the process to provide a clear picture of how intentions and beliefs relate.

What can cause an agent's database to change? In this paper, we focus on two main sources (figure~\ref{fig:dbperspective}):

\begin{enumerate}
\item The agent makes some observation, e.g. from sensory input. If the new observation is inconsistent with the agent's beliefs, these beliefs will have to be revised to accommodate it. While we are fully aware of their short- comings, in particular when it comes to iterated revision, our account of belief revision follows the classical AGM postulates~\citep{AGM1985} rather closely. The goal is thus to give general conditions on a single revision with new information that the agent has already committed to incorporating.
\item The agent forms a new intention. Here we focus on future directed intentions, understood as time-labeled actions pairs $(a,t)$ that might make up a plan. Analogously to belief revision, it is assumed the agent has already committed to a new intention, so it must be accommodated by any means short of revising beliefs. The force of the theory is in restricting how this can be accomplished. To be more precise, we purport to model an intelligent database, which receives instructions from some planner (e.g. a STRIPS-like planner) that is itself engaged in some form of practical reasoning. The job of the database is to maintain consistency and coherence between intentions and beliefs.
\end{enumerate}

This simple description, however, obscures some important subtleties in the interaction between beliefs and intentions. The following will serve as a running example that we will use frequently throughout the article.

\begin{example}[Running Example]
\label{expl:1}
Bobby the household robot is considering to buy groceries in the morning and to buy cleaning equipment in the afternoon. Although it is instructed to do both tasks, it only has sufficient budget to do either one of the two, but not both of them. Bobby thus believes it is possible to buy cleaning equipment and to buy food, but it also believes it is impossible to buy both. If Bobby decides to buy food, then it would like to cook in the afternoon.
\end{example}

Upon adopting the intention to buy food, Bobby will come to have new beliefs based on the predicted success of this intention, e.g., the he will be able to cook afterwards. These further beliefs are important when planning when or how to cook. The intention is also supported by the absence of certain beliefs. It would be irrational for Bobby to adopt the intention to buy food if it believed it did not have sufficient money. Likewise, even if it originally believed it has sufficient money, upon learning it does not, the intention to cook food should be dropped. Yet, when dropping this intention, other beliefs, such as that he will be able to cook, have to be dropped as well, which may in turn force other intentions and beliefs to be dropped. And so on. 

\subsection{Strong and weak beliefs}

To deal with these issues, we separate between beliefs depending on intentions, i.e. \emph{weak beliefs}, and beliefs that do not, i.e. \emph{strong beliefs}. Strong beliefs concern the world as it is, independent of the agent's future plans, but including what (sequences of) actions are possible. Thus, additionally to atomic facts, the agent may have beliefs about what the preconditions and postconditions of actions are, and about which sequences of actions are jointly possible.

A key element in our approach is that we treat preconditions of actions as \emph{assumptions}. This leads to an the asymmetry on beliefs about preconditions and postconditions of actions. First of all, we assume that 
\begin{quote}
\emph{If an agent intends to take an action, it weakly believes that its postconditions hold.}
\end{quote}
Since we are not considering actions whose effects are uncertain or dependent on the conditions that obtain when the action is taken, if an action is planned the planner believes whatever follows from it. 

However, for preconditions we add a weaker requirement:
\begin{quote}
\emph{If you intend to take an action you cannot believe that its preconditions do not hold}.
\end{quote}
This requirement is sometimes called \emph{strong consistency}, and is weaker than Bratman's \emph{means-end coherence} requirement~\cite{Bratman1987}. The result of this weakened requirement is that preconditions of actions are treated as \emph{assumptions}: An autonomous agent forms intentions under the assumption that these preconditions will be made true somewhere in the future. Treating preconditions as assumptions is a good fit with how real-time planning agents operate: Intended actions may be added as long as they are consistent with beliefs, and once they are accepted they can be used as additional assumptions to further plans~\citep{Shoham2009}. For instance, the household robot Bobby has the intention to cook diner tonight, which is based on the intention to buy the ingredients, which is in turn based on the assumptions that your friends will attend tonight, even if it does not know this for sure yet. It is only when Bobby finds out your friends are not coming, it should drop its intentions.

\iffalse
\subsection{The ``Little Nell'' problem: Not giving up too soon}
\label{sect:littlenell}

\cite{Mcdermott1982} discusses the following difficulty with a naive planning system:

\begin{quote}
Say a problem solver is confronted with the classic situation of a heroine, called Nell, having been tied to the tracks while a train approaches. The problem solver, called Dudley, knows that ``If Nell is going to be mashed, I must remove her from the tracks.'' (He probably knows a more general rule, but let that pass.) When Dudley deduces that he must do something, he looks for, and eventually executes, a plan for doing it. This will involve finding out where Nell is, and making a navigation plan to get to her location. Assume that he knows where she is, and he is not too far away; then the fact that the plan will be carried out will be added to Dudley's world model. Dudley must have some kind of database- consistency maintainer (Doyle, 1979) to make sure that the plan is deleted if it is no longer necessary. Unfortunately, as soon as an apparently successful plan is added to the world model, the consistency maintainer will notice that ``Nell is going to be mashed'' is no longer true. But that removes any justification for the plan, so it goes too. But that means ``Nell is going to be mashed'' is no longer contradictory, so it comes back in. And so forth.
\end{quote}

The agent continuously plans to save Nell, and abandons its plan because it believes it will be successful. If we view this problem from the database perspective, we require some way to separate beliefs about plans from beliefs that are not about plans. Otherwise, the planner may believe certain facts hold and adopt the plans accordingly, while these facts may be dependent on performing the plan.

This problem has been considered extensively in the literature (cf.~\cite{Cohen1990,Shoham2009,Icard2010,vanderHoek2003}). Our solution is to separate strong beliefs from weak beliefs. The beliefs in the belief database of the agent (those that will be used by the planner) are strong beliefs, and the weak beliefs are computed by adding intentions to the strong beliefs, and everything following from that.
\fi
\subsection{Results}
We develop a branching-time temporal logic, called \logicname{} (\logic{}) in order to formalize beliefs. The language of this logic contains formulas to reason about possibility, preconditions, postconditions, and the execution of actions. The semantics of this logic is close to CTL*, and in this way follows the tradition of BDI logics of~\cite{Rao1991}. An important difference is that we do not use modal operators to reason about time, but we use explicit time points. We axiomatize this logic and proof that the axiomatization is sound and strongly complete with respect to our semantics.

Secondly, we separate strong beliefs from weak beliefs as described above. Strong beliefs are beliefs that occur in the belief database, and they are independent of intentions. Weak beliefs are obtained from strong beliefs by adding intentions to the strong beliefs, and everything that follows from that. We then formalize a \emph{coherence condition} on the beliefs and intentions. This condition states that the agent weakly believes it is possible to jointly perform all of its intended actions. 

Thirdly, the main technical result of the paper is that we develop a set of postulates for the joint revision of belief and intentions, and that we prove a variation of the~\cite{Katsuno1991} representation theorem. To this end, we define a revision operator that revises beliefs up to a specific time point. We show that this leads to models of system behaviors which can be finitely generated, i.e. be characterized by a single formula.

\subsection{Map of the paper}

The structure of this paper is as follows. In section~\ref{sect:preliminaries} we discuss some background information on belief revision. The subsequent three sections are in line with our three main results: in section~\ref{sect:logic} we introduce and motivate our logic PAL, we axiomatize it and we proof completeness; in section~\ref{sect:intentions} we separate strong beliefs from weak beliefs, and we formalize a coherence condition on belief and intention; in section~\ref{sect:revision} we study revision of beliefs and intentions. In section~\ref{sect:applications} we discuss some applications of our revision operator. We discuss related work in both philosophy of mind and AI in section~\ref{sect:relatedwork}, and we provide directions for future work in section~\ref{sect:futurework}. All the proofs can be found in the appendix.

==> sections/iterated-revision_old.tex <==
\section{Iterated revision}
\label{sect:iterated-revision}

Until now we only considered single-step revision of belief and intention. In this part we develop an account of iterated revision by following the approach of~\cite{Darwiche1997} developed for propositional logic. They observe that the AGM postulates are too permissive to enforce plausible iterated revision. In order to remedy this, they suggest the following changes:
\begin{itemize}
\item Instead of performing revision on a propositional formula, perform revision on an abstract object called an \emph{epistemic state} $\Psi$, which contains the entire information needed for coherent reasoning.
\item Postulate (R4) is weakened as follows:

(R*4) If $\Psi=\Psi'$ and $\varphi\equiv\varphi'$, then $\Psi\circ\varphi\equiv\Psi'\circ\varphi'$
\item The following four desirable postulates are added for iterated revision:

(C1) If $\varphi\models\varphi'$, then $(\Psi\circ\varphi')\circ\varphi\equiv\Psi\circ\varphi$.

(C2) If $\varphi\models\neg\varphi'$, then $(\Psi\circ\varphi')\circ\varphi\equiv\Psi\circ\varphi$.

(C3) If $\Psi\circ\varphi\models\varphi'$, then $(\Psi\circ\varphi')\circ\varphi\models\varphi'$.

(C4) If $\Psi\circ\varphi\not\models\neg\varphi'$, then $(\Psi\circ\varphi')\circ\varphi\not\models\neg\varphi'$
\end{itemize}

We now provide the revision postulates from Definition~\ref{def:belief-intention-postulates}, but then for epistemic belief states. We also modify Postulate (P4) similar to how Darwiche and Pearl did.

\begin{definition}
\label{def:iterated-revision-postulatesA}
Postulates $(P^*1)-(P^*12)$ are obtained from $(P1)-(P12)$ (Definition \ref{def:belief-intention-postulates}) by replacing belief-intention databases with epistemic belief-intention databases, with the exception of $(P^*4)$ which relaxes $(P4)$ in the following way:\\
$(P^*4)$ If $\Psi=\Psi_2$ and $\varphi\equiv\varphi_2$ then $\Psi'\equiv\Psi_2'$.
\end{definition}

Similar to Section~\ref{sect:revision:postulates}, we define a bounded revision function up to a fixed time $t$, assuming that the strong beliefs and intentions in an epistemic belief-intention databases are all bounded up to $t$.

\begin{definition}[Epistemic belief-intention database]
\label{def:epistemic-belief-intention-database}
An \emph{epistemic belief-intention database} $(\Psi,I)$ consists of an epistemic state  $\Psi$, and an intention database $I$. The set of all epistemic belief-intention databases bounded up to $t$ is denoted by $\restebis{}$, or simply $\ebis{}$ if $t$ is clear from context.
\end{definition}

We define our operator for iterated revision. Note that $\Psi$ stands for $Bel(\Psi)$ whenever it is embedded in a propositional formula, and that $Bel(\Psi)$ is thus a set of strong beliefs. For example, we say that $(\Psi, I)$ is \emph{coherent} if $(Bel(\Psi), I)$ is coherent. Recall %from Definition~\ref{def:conventions} 
that we omit the temporal restriction superscript from sets if it is clear from context.

\begin{definition}[Iterated revision of epistemic belief-intention databases]
\label{def:iterated-revision-postulates} 
An \emph{epistemic belief-intention revision function} $\agr:\ebis{}\times (\sbel{}\times \ib{})\rightarrow \ebis$ maps an epistemic belief-intention database, a strong belief formula, and an intention--- all bounded up to $t$--- to an epistemic belief-intention database bounded up to $t$ such that:
\begin{itemize}

\item
Postulates $(P^*1)-(P^*12)$ (Definition~\ref{def:iterated-revision-postulatesA}) hold,
\item  if \\
$(\Psi,I)\agr(\varphi,i) = (\Psi',I')$,\\
$(\Psi,I_1)\agr(\varphi',i') = (\Psi'',I_1')$,\\
$(\Psi'',I_2)\agr(\varphi,i'')=(\Psi''',I_2')$,\\
then the following four postulates also hold:\\
%
$(C^*1)$ If $\varphi\models\varphi'$, then $\Psi'\equiv \Psi'''$\\
$(C^*2)$ If $\varphi\models \neg \varphi'$, then $\Psi'\equiv \Psi'''$\\
$(C^*3)$ If $\Psi'  \models\varphi'$, then $\Psi''' \models  \varphi'$\\
$(C^*4)$ If $\Psi'  \not\models\neg \varphi'$, then $\Psi''' \not\models  \neg\varphi'$
\end{itemize}
\end{definition}

Postulates (C*1)-(C*4) are simply (C1)-(C4) for our belief-intention revision operator. (C*1) states that if two beliefs are added, the first is redundant if the second one is more specific. In other words, only revising with the second belief would obtain the same belief set. (C*2) states that if the first belief is inconsistent with the second one, then revising with the first belief is unnecessary. (C*3) ensures that a belief should be retained when revising with another belief implies it. Finally, (C*4) states that if a belief $\varphi$ is not contradicted after revising with another belief $\varphi'$, then it should remain uncontradicted when the revising by $\varphi'$ is preceded by $\varphi$.

When switching from belief revision on a belief state to belief revision on an epistemic state the definition of a faithful assignment should be adopted accordingly. We will do this now for our setting.

\begin{definition}[Faithful assignment for iterated revision]
\label{def:tbounded:faithfulassigment:epst}
A \emph{$t$-bounded faithful assignment for iterated revision} is a function that assigns to each epistemic state $\Psi$ a total pre-order $\le_\Psi^t$ on all models,  and to each intention database $I\in \mathbb{ID}\rest{}$ a selection function $\sel$ (Definition \ref{def:selection-function}), such that the following conditions hold:

\begin{enumerate}
\item If $m_1,m_2\in Mod( \Psi)$, then $m_1\le_\Psi^t m_2$ and $m_2\le_\Psi^t m_1$
\item If $m_1\in Mod( \Psi)$ and $m_2\not\in Mod( \Psi)$, then $m_1<_\Psi^t m_2$
\item   $\Psi=\Phi$ only if $\le_\Psi=\le_\Phi$
\item If $\restt=T_2\rest{}$, then $(T,\pi)\le_\Psi^t (T_2,\pi_2)$ and $(T_2,\pi_2)\le_\Psi^t (T,\pi)$.

\smallskip


If $(\Psi,I)\agr(\varphi,i) = (\Psi',I')$, then


\item If $m_1\in Mod(\varphi)$ and $m_2 \in Mod(\varphi)$, then $m_1\le_\Psi^t m_2$ iff $m_1\le_{\Psi'}^tm_2$.

\item If $m_1\not\in Mod(\varphi)$ and $m_2\not \in Mod(\varphi)$, then $m_1\le_\Psi^t m_2$ iff $m_1\le_{\Psi'}^tm_2$.
\item If $m_1\in Mod(\varphi)$, $m_2\not \in Mod(\varphi)$ and $m_1<_\Psi^t m_2$, then $m_1<_{\Psi'}^tm_2$.
\item If $m_1\in Mod(\varphi)$, $m_2\not \in Mod(\varphi)$  and $m_1\le_\Psi^t m_2$, then $m_1\le_{\Psi'}^tm_2$.
\end{enumerate}
\end{definition}

The first four conditions are similar to the conditions on a faithful assignment for single-step revision (Definition~\ref{def:faithful-assignment}), with the difference that $\lept$ is replaced with $\le_\Psi^t$, and that Condition 3 has epistemic states in the antecedent instead of strong belief formulas. Conditions 5-8 are the semantic counterpart of (C*1)-(C*4).

\begin{theorem}[Representation Theorem for iterated revision]
\label{thm:singlestepA}
An epistemic belief-intention revision operator $*_t$ satisfies postulates $(P^*1)-(P^*12)$  and $(C^*1)-(C^*4)$  iff there exists a faithful assignment for iterated revision that maps each $\Psi$ to a total pre-order $\le_\Psi^t $ 
%such that 
%\begin{enumerate}
%\item[CR1] If $m_1\models\varphi$ and $m_2\models\varphi$, then $m_1\le_\Psi^t m_2$ iff $m_1\le_{\Psi*_t(\varphi,i)}^tm_2$, for every $i$.
%\item[CR2] If $m_1\not\models \varphi$ and $m_2\not\models \varphi$, then $m_1\le_\Psi^t m_2$ iff $m_1\le_{\Psi*_t(\varphi,i)}^tm_2$, for every $i$.
%\item[CR3] If $m_1\models\varphi$, $m_2\not\models\varphi$ and $m_1<_\Psi^t m_2$, then $m_1<_{\Psi*_t(\varphi,i)}^tm_2$, for every $i$.
%\item[CR4] If $m_1\models\varphi$, $m_2\not\models\varphi$ and $m_1\le_\Psi^t m_2$, then $m_1\le_{\Psi*_t(\varphi,i)}^tm_2$, for every $i$.
%\end{enumerate}
%
 and each $I$ to a selection function $\sel$
  such that if $(\Psi,I)*_t(\varphi,i)=(\Psi',I')$, then:
\begin{enumerate}
\item $Mod(\Psi')=\min(Mod(\varphi),\le_{\Psi}^t)$
\item $I' = \sel(Mod(Bel(\Psi')),i)$
\end{enumerate}
\end{theorem}

We next provide a concrete revision operator satisfying all the  postulates of Definition \ref{def:iterated-revision-postulates}, thus showing their \emph{consistency}.

Our operator is based on  Spohn's \emph{ordinal conditional ranking functions}, which can be seen as representations of epistemic states. For a given time $t$, our ranking function $\kappa_t$ deals with epistemic states of our logic in a similar way  as the operator based on Spohn's ranking function for propositional epistemic states, introduced in~\cite{Darwiche1997}. 

\begin{definition}[Spohn ranking function]
\label{def:spohnA}
A \emph{Spohn ranking function} $\kappa_t:\mods\rightarrow\timeflow{}$ assigns a rank to each model such that:

If $m_1=(T_1,\pi_1)$ and $m_2=(T_2,\pi_2)$ such that $T_1\rest{} = T_2\rest{}$, then $\kappa_t(m_1)=\kappa_t(m_2)$.\\

\noindent
We extend the ranking to propositions as follows: $$\kappa_t(\varphi)=\min_{m\models\varphi}\kappa_t(m).$$
\end{definition}

\begin{definition}[Accepted propositions]
\label{def:accepted-propositions}
Given a ranking function $\kappa_t$, the \emph{accepted propositions} $Bel(\kappa_t)$ are those for which the negation is implausible: $$Bel(\kappa_t) = \{\varphi\mid \kappa(\neg\varphi)>0\}.$$ 
\end{definition}

It follows that the models of these propositions are those which have rank 0: $$Mod(Bel(\kappa_t)) = \{m\mid \kappa_t(m)=0\}.$$ The fact that $Bel(\kappa_t)$ is a set of strong beliefs follows from the condition we put on the Spohn ranking function.

Now we define our revision operator. For the epistemic part  we follow~\cite{Darwiche1997}, while for intention revision we give prefer intentions that occur sooner rather than later.

\begin{definition}[Extended Spohn-based revision operator]
\label{def:spohn-iterated-revision-operator}
The \emph{Extended Spohn-based revision operator $\spohn$} is defined as follows:

$(\kappa_t,I)\spohn(\varphi,i) = (\kappa_t',I')$, where  $\kappa_t'$ and $I'$ are  such that\footnote{We show in the technical report that $\kappa_t'$ is a well defined   Spohn ranking function.}
\begin{align*}
\kappa_t'(m) = \begin{cases}
\kappa_t(m)-\kappa_t(\varphi), &\text{ if } m\models \varphi;\\
\kappa_t(m)+1,&\text{ if } m\models \neg \varphi,
\end{cases}
\end{align*}
%
and $I'$ is defined in the following iterative way. If $n$ is the maximal time instance that occurs in $I$, we define the sets of intentions

\begin{enumerate}
\item $I_{-1} =\{ i\}$, if $(Bel(\kappa_t'),\{ i \})$ is coherent, otherwise $I_{-1} = \emptyset$.
\item for every $\ell\in\{0,1,\dots,n\}$

\begin{enumerate}
\item if there is no $a$ such that $(a,\ell)\in I$, $I_{\ell} =I_{\ell-1}$.

\item otherwise, if $a$ is  the unique action such that $(a,\ell)\in I$, then  $I_{\ell} =I_{\ell-1}\cup\{ (a,\ell)\}$, if 
$(Bel(\kappa_t'),I_{\ell-1}\cup\{ (a,\ell)\})$ is coherent, otherwise $I_{\ell} =I_{\ell-1}$.

\end{enumerate}
\item $I'=I_n$.
\end{enumerate}

\end{definition}






We now pose our theorem.

\begin{theorem} The revision operator $\spohn$ satisfies postulates $(P^*1)-(P^*12)$ and $(C^*1)-(C^*4)$.
\end{theorem}

The Extended Spohn-based revision operator is an example of an operator satisfying the epistemic belief-intention revision function for iterated revision (Definition~\ref{def:iterated-revision-postulates}) and puts additional constraints on intentions. It prioritizes the new intention $i$, and after that it iteratively attempts to increase the set of new intentions by adding them in temporal order, starting with the most recent ones. We next give an example of how this may work in practice.

\begin{example}[Running example (Extended Spohn-based revision)]
Suppose\\  that 
Bobby the household robot has an epistemic  belief-intention database $EBI$ with intentions $I=\{(food, 0), (equip, 1)\}$, and suppose its epistemic state is formalized as:
\begin{itemize}
\item $\kappa_t(m) = 0$, for every $m\in Mod(\varphi_0)$, where
$$\varphi_0=\Box_0 pre(food, equip)_0$$ (``Bobby has precondition to buy both food and  cleaning equipment'')

\item $\kappa_t(m) = 1$,   for every $m\in Mod(\varphi_1)$, where
$$\varphi_1=\Box_0\neg pre(food,equip)_0\wedge \Box_0 pre(food)_0\wedge \Box_0 pre(equip)_1$$ (``Bobby  can carry  out any of two intended actions, but not both of them'')

\item $\kappa_t(m) = 3$,   for every $m\in Mod(\varphi_3)$, where
$$\varphi_3=\Box_0 \neg pre(food)_0 \wedge \Box_0 \neg pre(equip)_1$$ (``Bobby  cannnot carry  out any of two intended actions'')

\item $\kappa_t(m) = 2$,   for all other models, i.e., for  $m\in Mod(\varphi_2)$, where $\varphi_2=\neg\varphi_0\wedge\neg\varphi_1\wedge\neg\varphi_3$
%
(note that we can read $\varphi_2$ as ``Bobby  can buy only the cheaper of the two items'')

\end{itemize}
Thus, Bobby's beliefs are represented by $Bel(\kappa_t)$ (Definition~\ref{def:accepted-propositions}), which include that it believes it is possible to carry out both intended actions, so the agent is coherent. In addition, the epistemic state specifies a preference ordering over models as well, which is specified by the the ranking $\kappa$. It assumes that ``Bobby  cannnot carry  out any of two intended actions'' is the least plausible proposition.

Suppose next that Bobby revises its epistemic belief-intention database with\\
$(\Box_0\neg pre(food, equip)_0,\epsilon)$. The ranking function selects the minimal (i.e., the most plausible) model in which the revised formula is consistent, which has ranking 1. After revision, Bobby believes it is able to buy food or buy cleaning equipment, i.e., any of those two, but not both. The new ranking $\kappa'_t$ is as follows:
\begin{itemize}

\item $\kappa_t'(m) = 0$, for every $m\in Mod(\varphi_1)$

\item $\kappa_t'(m) = 1$,   for every $m\in Mod(\varphi_0\vee\varphi_2)$

\item $\kappa_t'(m) = 2$,   for every $m\in Mod(\varphi_3)$

\end{itemize}
The agent can then use $\kappa_t'$ for future revision. Using the intention revision operation of Definition~\ref{def:spohn-iterated-revision-operator}, it will keep the intention that it intends to carry out first, which means $I'=\{(food, 0)$, and the intention to buy cleaning equipment is dropped.
\end{example}

==> sections/multi-agent-system.tex <==
\section{Multi-agent system}
\label{sect:multi-agent-system}

In a multi-agent setting, revision of the beliefs and intentions of one agent may lead to the revision of intentions of other agents. For example, two household robots may jointly intend to move some furniture together at a specific time point in future. If one of the robots gets an urgent task that needs to be performed at that time point, or if one of the robots starts to believe that it has a malfunctioning part essential for moving heavy objects, then the joint intention of the second robot needs to be reconsidered. In this section, we consider such joint intentions as collective intention and assume that they can be reduced to a set of intentions of individual agents. Other (non-reducible) notions of collective intention, as studied in the literature of collective intentionality (see Section~\ref{sect:related-work:collective-intentions}) are left for further research.

\begin{figure}[h!]
\centering
  \centering \includegraphics[scale=0.5]{img/dbperspectivemas}
  \caption{A multi-agent system of belief-intention agents and a collective intention database}
  \label{fig:mas-overview}
\end{figure}

Collective intentions can be formed in various ways. They can be formed through communication and negotiation between agents, or they can be inserted by a central authority. Collective intentions are added to the collective intention database similar to how individual intentions are added to the individual intention databases. In general, we assume agents are engaged in some form of practical reasoning through which collective intentions are formed. The challenge that we consider in this section is to maintain the databases coherent. In our setting, a multi-agent system will consist of a set of agents coordinated through a collective intention database (Figure~\ref{fig:mas-overview}).

\noindent A collective intention database contains collective intentions of the form ``Agents $ag_1,\ldots,ag_n$ collectively intend to do $c$, and to this end agent $ag_1$ intends to take action $a_1$ at time $t_1$,\ldots, and agent $ag_n$ intends to take action $a_n$ at time $t_n$.'' The collective intention database captures two basic notions. First, it serves as a coordination mechanism for a set of agents by specifying what actions of the agents will be carried out together (but not necessarily at the same time moment), and in this way represents dependencies between the intentions of the individual agents. Secondly, it allows agents to reason about each others intentions, in the sense that each agent believes that the other agents will carry out their part in a collective intention, and if not, they will revise their intentions accordingly. That is, agents are committed to the collective intentions they participate in as long as they believe other agents will stay committed to their part as well.

\begin{example}[Running example (Ctd.)]
Two household robots, Annie ($ag_1$) and Bobby ($ag_2$), are planning tasks that they will carry out for their owner throughout the day. There are several tasks, some of which have to be carried out together. The individual tasks are to clean the house ($clean$) and to fetch the newspaper ($fetch$), and the collective tasks are to make breakfast (i.e. prepare breakfast ($prep$) and bring breakfast ($bring$)) and to move some heavy furniture ($move$).

The specification of the individual and collective intentions of the agents after a process of individual and collective deliberation is depicted in Figure~\ref{fig:specification}. As can be read from the figure, Annie intends to first fetch the newspaper, then bring the breakfast, and finally move the furniture. Bobby intends to first prepare breakfast, then clean the house and finally move the furniture. The dashed lines in the figure indicate collective intentions. The collective intention to make breakfast consists of Bobby preparing breakfast at time 0, and Annie bringing the breakfast to the owner at time 1. The collective intention to move a heavy piece of furniture consists of both agents moving the furniture at time 2.

\begin{figure}[h!]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,
  main node/.style={circle,draw,font=\sffamily\small},dotted node/.style={circle,fill=white,font=\sffamily\small},pi node/.style={circle,fill=white,font=\sffamily\Large}]

   \node[dotted node] (ag10) {Annie ($ag_1)$:};
   \node[dotted node] (ag11) [right=0.2cm of ag10] {$t_0$};
   \node[dotted node] (ag12) [right=1.5cm of ag11] {$t_1$};
   \node[dotted node] (ag13) [right=1.5cm of ag12] {$t_2$};
   \node[dotted node] (ag14) [right=1.5cm of ag13] {$t_3$};
   \node[dotted node] (ag20) [below=0.3cm of ag10]    {Bobby ($ag_2$):};
   \node[dotted node] (ag21) [right=0.2cm of ag20] {$t_0$};
   \node[dotted node] (ag22) [right=1.5cm of ag21] {$t_1$};
   \node[dotted node] (ag23) [right=1.5cm of ag22] {$t_2$};
   \node[dotted node] (ag24) [right=1.5cm of ag23] {$t_3$};
   
   
  \path[every node/.style={font=\sffamily\small}]
    (ag11) edge node [sloped,anchor=center,above] {fetch} (ag12)
    (ag12) edge node [sloped,anchor=center,above] {bring} (ag13)
    (ag13) edge node [sloped,anchor=center,above] {move} (ag14)
    (ag21) edge node [sloped,anchor=center,above] {prep} (ag22)
    (ag22) edge node [sloped,anchor=center,above] {clean} (ag23)
    (ag23) edge node [sloped,anchor=center,above] {move} (ag24)
    ;
      \draw [dashed, -] ($ (ag13) + (1.1,0.05) $) -- ($ (ag23) + (1.1,0.5) $);
      \draw [dashed,-] ($ (ag12) + (1.1,0.05) $) -- ($ (ag21) + (1.2,0.5) $);
    
\end{tikzpicture}
\caption{Individual and collective intentions of Annie and Bobby.}
\label{fig:specification}
\end{figure}
\end{example}

\subsection{\maslogic{}: a logic for multi-agent beliefs and intention}
\label{sect:mas:logic}

We only provide a brief summary of our extension here. More details can be found in the technical report.

\maslogic{} is used to model the belief base of a single agent in a multi-agent system. The logic is a straightforward generalization of \logic{}, introduced in Section \ref{sect:logic}. Suppose a finite set of agents  $\ag{}=\{ag_1,\ldots, ag_n\}$. As before, $\act{}=\{a,b,c,\ldots\}$ is a finite set of deterministic primitive actions.
We assume that actions in multi-agent systems are executed concurrently. For that reason, we consider the set of \emph{action profiles} $\actp{} = \act{}^n$. For $\{a_1,\ldots,a_n\}\subseteq \act{}$ and $\alpha=(a_1,\dots,a_n)\in \actp{}$, we assume that the agent $ag_k$ executes the action $a_k$, for every $ag_k\in \ag{}$.
 
The language $\maslang{}$ of the logic \maslogic{} is defined in a similar way as the language $\lang{}$ of PAL  (Definition \ref{def:language}). The difference is that now the preconditions and postconditions are defined for action profiles, i.e., the  set of primitive propositions is the finite set $$\prop{}_{MAS}=\{p,q,r,\ldots\}\cup \{pre(\overline{\alpha}), post(\alpha)\},$$ where $\overline{\alpha}=(\alpha_1,\alpha_2,\ldots,\alpha_m)$ is a non-empty sequence of action profiles and $\alpha\in \actp{}$ is an action profile. As before, we denote primitive propositions with $\chi$.
We use those propositions to define the formulas of our language as $$\varphi ::= \chi_t\mid do(\alpha)_t\mid\Box_t\varphi\mid\varphi\wedge\varphi\mid\neg\varphi,$$
with $\chi\in \prop{}_{MAS}, \alpha\in \actp{}$ and $t\in\mathbb{N}$.

The semantics of PALM is the same as PAL, except that the state transitions are labeled with action profiles rather than actions.

\begin{example}[Running Example (Ctd.)]
An example model is shown in Figure~\ref{fig:example:mas-tree}. For clarity, the valuation function is not visualized but we could for instance have that $pre(fetch,prep)\in s_0$ and $post(fetch,prep)\in s_1$.
\end{example}

\begin{figure}[h!]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,
  thick,main node/.style={circle,draw,font=\sffamily\small\bfseries},dotted node/.style={circle,fill=white,font=\sffamily\tiny\bfseries},pi node/.style={circle,fill=white,font=\sffamily\Large\bfseries}]

   \node[main node]   (s0) {$s^0$};
  \node[main node]   (s1) [above right=0.3cm and 1.9cm of s0] {$s^1$};
  \node[dotted node] (d1) [right=1.9cm of s0] {\ldots};
  \node[main node]   (s2) [below right=0.3cm and 1.9cm of s0] {$s^2$};
  \node[dotted node] (d2) [right=0.3cm and 1.9cm of s2] {\ldots};
  \node[main node]   (s3) [above right=0.3cm and 1.9cm of s1] {$s^3$};
  \node[dotted node] (d3) [right=1.9cm of s1] {\ldots};
  \node[main node]   (s4) [below right=0.3cm and 1.9cm of s1] {$s^4$};
  \node[main node]   (s5) [below right=0.3cm and 1.8cm of s2] {$s^5$};
  \node[main node]   (s6) [above right=0.3cm and 1.9cm of s3] {$s^6$};
  \node[main node]   (s7) [above right=0.3cm and 1.9cm of s4] {$s^7$};
  \node[main node]   (s8) [below right=0.3cm and 1.9cm of s4] {$s^8$};
  \node[main node]   (s9) [below right=0.3cm and 1.9cm of s5] {$s^9$};
  \node[pi node] (pi1) [right=0.05cm of s6] {$\pi_1$};
  \node[pi node] (pi2) [right=0.05cm of s7] {$\pi_2$};
  \node[pi node] (pi3) [right=0.05cm of s8] {$\pi_3$};
  \node[pi node] (pi4) [right=0.05cm of s9] {$\pi_4$};
  \node[dotted node] (d5) [right=2cm of s5] {\ldots};
  \path[every node/.style={font=\sffamily\scriptsize}]
    (s0) edge node [sloped,anchor=center,above] {(fetch,prep)} (s1)
    (s1) edge node [sloped,anchor=center,above] {(bring.clean)} (s3)
    (s1) edge node [sloped,anchor=center,above] {(bring.NOP)} (s4)
    (s0) edge node [sloped,anchor=center,above] {(fetch,NOP)} (s2)
    (s3) edge node [sloped,anchor=center,above] {(move,move)} (s6)
    (s2) edge node [sloped,anchor=center,above] {(bring,clean)} (s5)
    (s4) edge node [sloped,anchor=center,above] {(move,NOP))} (s7)
    (s4) edge node [sloped,anchor=center,above] {(NOP,move))} (s8)
    (s5) edge node [sloped,anchor=center,above] {(move,move)} (s9)
    ;    
\end{tikzpicture}
\caption{Example tree $T$ with paths $\pi_1$ to $\pi_4$}
\label{fig:example:mas-tree}
\end{figure}

\subsection{Adding collective intentions}
In order to formalize the dependencies between agents that collective intentions induce, we introduce a collective intention database. Similar to the individual intentions, collective intentions also should be non-overlapping for a single agent.

\begin{definition}[Collective intention database]
A collective intention $c$ is a set consisting of triples of the form $(ag_k,a,t)$, where $ag_k\in\ag{}, a\in\act{}$, and $t\in\mathbb{N}$. A \emph{collective intention database} $C=\{c_1,\ldots,c_m\}$ is a set of collective intentions that do not overlap, i.e., 
$$\text{for each } (ag_k,a, t)\in \bigcup C: \text{if } a\not=b\text{, then } (ag_k,b, t)\notin \bigcup C.$$
We denote the set of all collective intention databases with $\mathbb{CID}$.
\end{definition}

We assume agents $ag_1,\ldots,ag_n$ and we define a multi-agent system consisting of belief-intention databases $(SBM_k,I_k)$ for each agent $ag_k$, and a collective intention database. We make this precise in the following definition.

\begin{definition}[Multi-agent system]
\label{def:mas}
Let $SBM$ be a set of strong beliefs in PALM and let $Ag=\{ag_1,\ldots,ag_n\}$.

A \emph{multi-agent system} $(AGT,C)$ consists of a tuple of belief-intention databases $AGT = \langle (SBM_1,I_1),\ldots,(SBM_n,I_n)\rangle$ and a collective intention base $C$ such that the collective and individual intentions are non-overlapping, i.e.: $$\text{for each } (ag_i,a, t)\in \bigcup C: \text{if } a\not=b\text{, then } (b,t)\not\in I_i.$$
\end{definition}

For each agent, we specify a ``view'' on the collective intention database, which contains the collective intentions in which an agent participates and the agent's individual intentions. They are collected in a set of triples, which simplifies the notation of the weak beliefs and the coherence condition later on.

\begin{definition}[Intention view]
\label{sect:collective-intention-view}
The \emph{ intention view} %$V_k =V(I_k,C)$ 
for an agent $ag_k$ in the multi-agent system $ (\langle (\psi_1,I_1), \ldots,(\psi_n,I_n) \rangle,C)$ is defined as:
\begin{align*}
V_k = \bigcup\{c\in C \mid (\exists a\in \act )(\exists t\in \mathbb N). (ag_k,a,t)\in c \}\cup \{(ag_k,a,t)\mid (a,t)\in I_k\}.
\end{align*}
\end{definition}

\begin{example}[Running example (Ctd.)]
The multi-agent system of our households robots is $(AGT,C)$, where $AGT=\langle(SBM_1,I_1), (SBM_2, I_2)\rangle$ and $C=\{c_1,c_2\}$ such that:
\begin{flalign*}
&\qquad I_1=\{(fetch,0)\}&\\
&\qquad I_2=\{(clean,1)\}&\\
&\qquad c_1=\{(ag_1,bring,1),(ag_2,prep,0)\}&\\ 
&\qquad c_2=\{(ag_1,move,2),(ag_2,move,2)\}&
\end{flalign*}
%
The intention views for both agents are as follows:

\smallskip


%\begin{itemize}
%\item 
\noindent $V_1=\{(ag_1,fetch,0),(ag_2,prep,0),(ag_1,bring,1),(ag_1,move,2),(ag_2,move,2)\}$,

\smallskip

%\item 
\noindent $V_2=\{(ag_2,prep,0),(ag_1,bring,1),(ag_2,clean,1),(ag_1,move,2),(ag_2,move,2)\}$.
%\end{itemize}
\end{example}

In the single-agent case, weak beliefs are obtained from strong beliefs by adding intended actions and everything that follows from that (Definition~\ref{def:weak-beliefs}). In the multi-agent case, the collective intentions in which the agent participates are added to this as well. 

\smallskip

\noindent\emph{Notation:} Given an action profile $\beta=(b_1,\ldots,b_n)$, $\beta^k$ denotes the k'th action of $\beta$, i.e., $\beta^k=b_k$, and $(a,\beta^{-k})$ denotes the action profile $\beta$ in which action $\beta^k$ is replaced with action $a$, i.e.,  $(a,\beta^{-k})=(b_1,\ldots,b_{k-1},a,b_{k+1}\ldots,b_n)$.

\begin{definition}[Weak beliefs in \maslogic{}]
\label{def:weak-beliefs-mas}
 Given a \emph{multi-agent system} $(AGT,C)$, with $AGT=\langle(SBM_1,I_1),\ldots,(SBM_n,I_n)\rangle$, the weak beliefs for agent $ag_k$ are defined as follows: $$WB(SBM_k, V_k) = Cn(SBM_k\cup \{\bigvee_{\beta\in\actp{}} do(a, \beta^{-k})_t\mid (ag_m,a,t)\in V_k\},$$
where $V_k$ is the intention view for agent $ag_k$ (Definition~\ref{sect:collective-intention-view}).
\end{definition}

The disjunction in the definition above entails that the agent draws inferences from its intentions if they are true in some contingent futures, regardless of what the other agents do. This is in line with the weak conditions on commitments in the single-agent case (see Remark~\ref{remark:pissofdragan}). We will show this in more detail in the following examples.

\begin{example}[Weak beliefs in PALM]
Suppose $Act = \{a, b\}$, and agent $ag_1$ and $ag_2$ in a multi-agent system $(\langle(SBM_1,I_1), (SBM_2,I_2)\rangle, C)$. Furthermore $I_1 = \{(a,2)\}$, and $C = \{c_1, c_2\}$, where
\begin{itemize}
\item $c_1 = \{(ag_1, a, 0), (ag_2, b, 2)\}$,
\item $c_2 = \{(ag_1, b, 1), (ag_2, a, 5)\}$.
\end{itemize}
The intention view for agent $ag_1$ is:
\begin{itemize}
\item $V_1 = \{(ag_1,a,0),(ag_1,b,1),(ag_1,a,2),(ag_2,b,2),(ag_2,a,5)\}$.
\end{itemize}
The weak beliefs for agent $ag_1$ are then as follows:
$$WB(SBM_1, V_1) = Cn(SBM_1\cup \Theta),$$
where,
\begin{align*}
\Theta = \{&do(a, a)_0\vee do(a,b)_0, do(b,a)_1\vee do(b,b)_1,\\
&do(a,a)_2\vee do(a,b)_2,do(a,b)_2\vee do(b,b)_2,\\
&do(a,a)_5\vee do(b,a)_5\},
\end{align*}
which simplifies to:
\begin{align*}
\Theta = \{&do(a, a)_0\vee do(a,b)_0, do(b,a)_1\vee do(b,b)_1,\\
&do(a,b)_2, do(a,a)_5\vee do(b,a)_5\},
\end{align*}
\end{example}

\begin{example}[Running example (Ctd.)]
For our running example, recall that for agent $ag_1$ the intention view is as follows:
\begin{itemize}
\item $V_1=\{(ag_1,fetch,0),(ag_2,prep,0),(ag_1,bring,1),(ag_1,move,2),(ag_2,move,2)\}$.
\end{itemize}
%
The weak beliefs of agent $ag_1$ are $WB(SBM_1, V_1) = Cn(SBM_1 \cup \Theta)$, where:
\begin{align*}
\Theta =& \{\bigvee_{b\in\act{}} do(a,b)_t\mid (ag_i,a,t)\in V_1\}\\
     =&\{do(fetch,prep)_0, \bigvee_{b\in\act{}} do(bring,b)_1, do(move,move)_2\}.
\end{align*}
\end{example}

We next define the coherence condition for an agent in the multi-agent system. Similar to the idea of weak beliefs, the beliefs of an agent should not only be coherent with its own intentions, but they should also be coherent with some of the intentions of other agents. An agent is coherent in the multi-agent system if it considers it possible 1) to carry out all of its individual intentions, 2) to carry out its part in all the collective intentions in which it participates, and 3) for all other agents in these collective intentions to carry out their intentions as well. This means that the agent is \emph{committed to its intentions} as long as it doesn't believe they are impossible. While in the single-agent case this was dependent only on its own actions, in the multi-agent case this is dependent on the actions of other agents as well. In other words, the agents assumes commitment of the other agents.

\begin{definition}[Coherence condition in multi-agent system]
\label{def:coherence-multiagent} 
Given an intention view $V_k$ (Definition~\ref{sect:collective-intention-view}), let $t_{\min}$ and $t_{\max}$ be the minimal and maximal time component occurring in $V_k$. Then\footnote{Recall that $\alpha^m$ denotes the $m$'th action in the action profile $\alpha$. $\alpha_x$ does not denote a single action, but refers to the $x$'th action profile in a sequence of action profiles.}
\begin{flalign*}
Cohere(V_k) = \Diamond_0\bigvee_{\alpha_{t_x}^m=b_{t_x} :  (ag_m,b_{t_x},t_x)\in V_k} pre(\alpha_{t_{\min}},\alpha_{t_{\min+1}},\ldots,\alpha_{t_{\max}})_{t_{\min}}.
\end{flalign*}

A pair $(SBM,V)$ consisting of a set of strong beliefs $SBM$ and an intention view $V$ is \emph{coherent} iff $SBM$ is consistent with $Cohere(V) $, i.e., $SBM\not\vdash\neg Cohere(V)$.\footnote{Similar to the single-agent case, we can define coherence semantically in a similar way due to the completeness theorem.}
\end{definition}

The subscript of the disjunction in the coherence condition of Definition~\ref{def:coherence-multiagent} takes into account each element $(ag_m,b_{t_x},t_x)$ from the intention view $V_k$, and fixes the corresponding action $b_{t_x}$ of the agent $ag_m$ at the coordinate $m$ of the action profile $\alpha_{t_x}$ in the corresponding time point $t_x$. Here the actions of $ag_k$ from the intention view are fixed, but also the actions from $V_k$ of the other agents. The disjunction allows the remaining actions in the action profiles to range over $\act{}$.

We illustrate this definition with a simple example.

\begin{example}[Multi-agent coherence condition]
For the set of actions $\act{}=\{a,b,c\}$, let $(AGM,C)$ be a multi-agent system such that $AGM=\langle(SBM_1,I_1),(SBM_2,I_2)\rangle$ and $I_1=\{(a,1)\}$. Suppose furthermore that the collective database is $$C=\{\{(ag_1,b,2),(ag_2,c,1)\},\{(ag_1,c,3),(ag_2,a,3)\}\}.$$ The intention view of agent $ag_1$ is as follows: $$V_1 = \bigcup C \cup \{(ag_1,a,1)\}.$$
Then
\begin{flalign*}
Cohere(V_1) = \Diamond_0\bigvee_{\alpha^2=c,\beta^2\in\act{},\gamma^2=a} pre(\alpha,\beta,\gamma)_{1}, \ \  \textit{i.e.,}
\end{flalign*}
%
$Cohere(V_1) = \Diamond_0( pre(\alpha',(b,a),\gamma')_{1} \vee  pre(\alpha',(b,b),\gamma')_{1} \vee  pre(\alpha',(b,c),\gamma')_{1},$

\smallskip

where $\alpha'=(a,c),\gamma'=(c,a)$.

\end{example}

In the technical report, we show that coherence of beliefs and an intention view implies joint consistency of the beliefs and intentions from the view.

\subsection{Multi-agent revision}

The revision postulates and a representation theorem for multi-agent revision can be found in the technical report. Here we explain the intuitions. 

Similarly as in the single-agent case, we use belief formula $\psi_k$ instead of $SBM_k$. We define two new revision operators for a multi-agent system $(AGM, C)$ with agents $ag_1,\ldots,ag_n$ and $AGM=\langle(\psi_1,I_1),\ldots,(\psi_n,I_n)\rangle$: 
\begin{itemize}
\item A \emph{multi-agent revision function} $\agrk$, which revises agent $ag_k$ with the pair $(\varphi, i$), consisting of a strong belief formulas $\varphi$ from PALM and an intention $i$, all bounded up to $t$: $$(AGM,C)\agrk(\varphi,i)=(AGM',C'),$$ 
where $AGM'=\langle(\psi_1',I_1'),\ldots,(\psi_n',I_n')\rangle$. This function has the following properties:
\begin{itemize}
\item For all $(\psi_j, I_j)$ with $j\not=k$: $\psi_j'=\psi_j$ and $I_j'=I_j$: Revision of a single agent in the multi-agent system does not affect the strong beliefs or individual intentions of the other agents,
\item Similar to the single-agent case, the agent first revises its strong beliefs using the AGM postulates, and then its intentions,
\item $(\psi_j',V_j')$ is coherent according to Definition~\ref{def:coherence-multiagent} for all $j$: All agents should be coherent after revision,
\item If possible, $i\in I_k$. This may require dropping individual intentions of $ag_k$ or collective intentions in which agent $ag_k$ participates (see Example~\ref{example:mas-revision1}).
\end{itemize} 
\item A \emph{collective intention revision function} $\otimes$, which revises the multi-agent system with a collective intention $c$: $$(AGM,C)\otimes c = (AGM',C'),$$
where $AGM'=\langle(\psi_1',I_1'),\ldots,(\psi_n',I_n')\rangle$. This function has the following properties:
\begin{itemize}
\item $\psi'_j=\psi_j$ for all $j$: Revision of collective intentions does not revise the strong beliefs of individual agents,
\item $(\psi_j',V_j')$ is coherent according to Definition~\ref{def:coherence-multiagent} for all $j$: All agents should be coherent after revision,
\item If possible, $c\in C'$. This may require dropping individual or collective intentions that were dependent on $c$ (see Example~\ref{example:mas-revision2}).
\end{itemize}
\end{itemize}

We end with two examples illustrating how these revision operators may work in practice.

\begin{example}[Running example, individual revision]
\label{example:mas-revision1}
Recall the multi-agent system $(AGT, C)$ of our example with $AGT=\langle(\psi_1,I_1),(\psi_2,I_2)\rangle$ and $C=\{c_1,c_2\}$ is formalized as follows:
\begin{flalign*}
&\qquad I_1=\{(fetch,0)\}&\\
&\qquad I_2=\{(clean,1)\}&\\
&\qquad c_1=\{(ag_1,bring,1),(ag_2,prep,0)\}&\\ 
&\qquad c_2=\{(ag_1,move,2),(ag_2,move,2)\}&
\end{flalign*}
Suppose furthermore that $ag_2$ believes it is only possible to move the furniture if it cleans the house before, i.e.,
\begin{align}
\label{formula-mas-revision}
\psi_2=\Box_0(\big(\bigvee_{a\in \act{}} post(a, clean)_2\big) \leftrightarrow pre(move,move)_2).
\end{align}
Now suppose $ag_2$ learns it is no longer possible to clean the house: $$(AGT,C)\agr^2 (\neg\Diamond_0 \bigvee_{a\in\act} pre(a, clean)_1, \epsilon) = (AGT',C'),$$
where $AGT'=\langle(\psi_1',I_1'),(\psi_2',I_2')\rangle$. Since the new belief is consistent with $\psi_2$, $\psi_2'$ is simply the conjunction of the old belief and the new belief. To remain coherent (Definition~\ref{def:coherence-multiagent}), agent $ag_2$ has to drop the intention $(clean,1)$, but it also has to drop its intention to move the furniture because the precondition is no longer satisfied ($\psi_2'$ implies $\Box_0\neg  pre(move,move)_2$). However, since this intention is part of a collective intention, $ag_1$ also drops its part and as a result collective intention $c_2$ is dropped. The situation after revision is thus as follows:
\begin{flalign*}
&\qquad I_1'=\{(fetch,0)\}&\\
&\qquad I_2'=\emptyset&\\
&\qquad C' = \{c_1\}&
\end{flalign*}
\end{example}


\begin{example}[Running example, collective intention revision]
\label{example:mas-revision2}
We continue with the situation after revision of the previous example. Suppose that after some deliberation, it turns out that the owner of Annie and Bobby is having some friends over for lunch. As a result, the collective intention for the household robots to make lunch at time 2 is added: $$(AGT',C')\otimes c_3 = (AGT'',C''),$$
where $c_3=\{(ag_1,cook, 2), (ag_2,cook,2)\}$.
However, $ag_2$ believes that there is only sufficient food left to either make breakfast at time 0, or to cook lunch at time 2. Since the newly added collective intention is preferred over the existing one, the other collective intention is dropped. The situation after revision is thus as follows:
\begin{flalign*}
&\qquad I_1''=\{(fetch,0)\}&\\
&\qquad I_2''=\emptyset&\\
&\qquad C'' = \{c_3\}&
\end{flalign*}
This means that the household robots won't prepare the owner breakfast, but instead cook lunch for the guests afterwards.
\end{example}

==> sections/revision_old.tex <==
\section{Revision of belief and intention}
\label{sect:revision}
In this section we turn to the {\em dynamic} part of our belief-intention databases by studying the revision of belief and intention. We provide and motivate a set of revision postulates on a belief-intention database $(SB,I)$ in Section~\ref{sect:revision:postulates}, and we prove our main representation theorem in Section~\ref{sect:revision:representation}. We discuss various examples in Section~\ref{sect:examples}.

The challenge of obtaining our result is two-fold:
\begin{itemize}
\item When revising a belief database that is bounded up to some time $t$ with a strong belief, we have to ensure that the resulting belief database is also bounded up to $t$,
\item When revising a belief database we also have to ensure the new belief database remains a strong belief. 
\end{itemize}

Our solution to is to bound both the syntax of \logic{} and the revision operator up to some time $t$ in the first subsection. In the second subsection we do the same for the semantics.

\subsection{Preliminaries: Belief Revision}
\label{sect:preliminaries}
The AGM postulates~\citep{AGM1985} formulate properties that should be satisfied by any (rational) revision operators defined on deductively closed sets of propositional formulas.~\cite{Katsuno1991} represent a belief set $B$ as a propositional formula $\psi$ such that $B=\{\varphi\mid\psi\vdash\varphi\}$. They define the following six postulates for revision on $\psi$ and show that these are equivalent to the eight AGM postulates:\\
\begin{enumerate}
\item[(R1)]
$\psi\br\varphi$ implies $\varphi$
\item[(R2)]
If $\psi\wedge\varphi$ is satisfiable, then $\psi\br\varphi\equiv\psi\wedge\varphi$
\item[(R3)]
If $\varphi$ is satisfiable, then $\psi\br\varphi$ is also satisfiable
\item[(R4)]
If $\psi\equiv\psi'$ and $\varphi\equiv\varphi'$, then $\psi\br\varphi\equiv\psi'\br\varphi'$
\item[(R5)] $(\psi\br\varphi)\wedge \varphi'$ implies $\psi\br(\varphi\wedge\varphi')$
\item[(R6)] If $(\psi\br\varphi)\wedge\varphi'$ is satisfiable, then $\psi\br(\varphi\wedge\varphi')$ implies $(\psi\br\varphi)\wedge\varphi'$
\end{enumerate}

Given a set $\mathbb{J}$ of all interpretations over some propositional language, they define a faithful assignment as a function that assigns each $\psi$ to a pre-order $\le_\psi$ on models satisfying the following three conditions:
\begin{enumerate}
\item If $J,J'\in Mod(\psi)$, then $J<_\psi J'$ does not hold.
\item If $J\in Mod(\psi)$ and $J'\not\in Mod(\psi)$, then $J<_\psi J'$ holds.
\item If $\psi\equiv\phi$, then $\le_\psi = \le_\phi$.
\end{enumerate}

They show in a representation theorem that a revision operator $\circ$ satisfies postulates (R1)-(R6) iff there exists a faithful assignment that maps each formula $\psi$ to a total preorder $\le_\psi$ such that 
\begin{align*}
Mod(\psi\circ\varphi) = \min(Mod(\varphi),\le_\psi).
\end{align*}

\subsection{Revision postulates} 
\label{sect:revision:postulates}

Recall from Section~\ref{sect:preliminaries} that we aim to prove a representation theorem comparable to that of~\cite{Katsuno1991}. Therefore, we follow their convention to fix a way of representing a belief set $SB$ consisting of strong beliefs by a single strong belief formula $\psi$ such that $SB=\{\varphi\mid\psi\vdash\varphi\}$. One of the main difficulties in this respect is that time in \logic{} is infinite in the future, so it is generally not possible to represent $SB$ closed under consequence by a single formula $\psi$, since this may potentially lead to an infinite conjunction. Therefore, we cannot prove the Katsuno and Mendelzon representation theorem directly. In this section, we define a \emph{bounded} revision function and we restrict the syntax of \logic{} up to a specific time point.

We first define some notation that we use in the rest of this section.

\paragraph{Notation}
\begin{itemize}
\item
By slight abuse of terminology, a pair $(\psi,I)\in\sbel\times \idb$ consisting of a strong belief formula $\psi$ and an intention database $I$ is also called a \emph{belief-intention database},
\item For $\varphi,\psi\in \sbel$, we write $\varphi\equiv\psi$ to denote that $\vdash \varphi\leftrightarrow\psi$,
\item $\epsilon$ is the special ``empty'' intention.
\item We denote $\bis{},\sbel{},\ib{}$, and $\idb$ bounded up to $t$ with respectively $\bis\rest{}, \sbel{}\rest{}, \ib{}\rest{}$, and $\idb\rest{}$. However, if the restriction is clear from context, we may omit the superscript notation. 
\end{itemize}

In the next definition we define a bounded revision function $\agr$ revising a belief-intention database $(\psi,I)$ with a tuple $(\varphi,i)$ consisting of a strong belief $\varphi$ and an intention $i$, denoted $(\psi,I)\agr(\varphi,i)$, where $t$ is the maximal time point occurring in $\psi, I, \varphi$, and $i$. 

A planning agent can seek some information while finding a plan (e.g. train time table) and then return both a new intention and the beliefs on which it is based. There are interactions between beliefs and intentions when revising. If we revise with only a belief then we may still require revision of intentions, so our revision procedure consists of revising with a belief and an intention simultaneously. We choose this since it captures the interactions between beliefs and intentions more closely.

\begin{remark}
We will define a single revision function, revising by a pair $(\varphi,i)$. Our approach allows one to define separate revision as well:
\begin{itemize}
\item Revising by $(\varphi,\epsilon)$ mirrors revising by a strong belief $\varphi$ and no intention,
\item Revising by $(\top,i)$ mirrors revising by no belief and an intention $i$.
\end{itemize}
We will show in Example~\ref{expl:jointvsseparaterevision} that there are situations in which it is more desirable to revise with a pair $(\varphi,i)$ instead of first revising with $(\varphi,\epsilon)$ and then with $(\top,i)$, since it avoids throwing away intentions unnecessarily.
\end{remark} 

\begin{definition}[Belief-intention revision function]\label{def:belief-intention-postulates} 
A \emph{belief-intention revision function} $\agr:\bis{}\times (\sbel{}\times \ib{})\rightarrow \bis$ maps a belief-intention database, a strong belief formula, and an intention--- all bounded up to $t$--- to a belief-intention database bounded up to $t$ such that if, \\
$(\psi,I)\agr(\varphi,i) = (\psi',I')$,\\
$(\psi_2,I_2)\agr(\varphi_2,i_2)=(\psi_2',I_2')$,\\
then following postulates hold:\\
$(P1)$ $\psi'\vdash\varphi$.\\
$(P2)$ If $\psi\wedge\varphi$ is satisfiable, then $\psi'\equiv \psi\wedge\varphi$.\\
$(P3)$ If $\varphi$ is satisfiable, then $\psi'$ is also satisfiable.\\
$(P4)$ If $\psi\equiv\psi_2$ and $\varphi\equiv\varphi_2$ then $\psi'\equiv\psi_2'$.\\
$(P5)$ If $\psi\equiv\psi_2$ and $\varphi_2\equiv \varphi\wedge\varphi'$ then $\psi'\wedge\varphi'$ implies $\psi_2'$.\\
$(P6)$ If $\psi\equiv\psi_2$, $\varphi_2\equiv \varphi\wedge \varphi'$, and $\psi'\wedge\varphi'$ is satisfiable,\\
\hspace*{2cm}then $\psi_2'$ implies $\psi'\wedge\varphi'$.\\
$(P7)$ $(\psi',I')$ is coherent.\\
$(P8)$ If $(\psi',\{i\})$ is coherent, then $i\in I'$.\\
$(P9)$ If $(\psi',I\cup\{i\})$ is coherent, then $I\cup\{i\}\subseteq I'$.\\
$(P10)$ $I'\subseteq I\cup \{i\}$.\\
$(P11)$ If $I=I_2$, $i=i_2$, and $\psi'\equiv\psi_2'$, then $I'=I_2'$.\\
$(P12)$ For all $I''$ with $I'\subset I''\subseteq I\cup\{i\}$:$(\psi',I'')$ is not coherent.
\end{definition}

Postulates (P1)-(P6) are the~\cite{Katsuno1991} postulates in our setting, which are equivalent to the AGM postulates. They also state that the revision of strong beliefs does not depend on the intentions. This can also be witnessed by the fact that all postulates involving intentions, i.e. (P7)-(P12), only use the revised strong belief formula $\psi'$. Therefore, revising strong beliefs does not depend on which intentions an agent had, or which intention it revises with. However, revising intentions \emph{does} have an effect on the weak beliefs (see the last paragraph of Example~\ref{expl:addingintention}). In other words, the procedures runs as follows:
\begin{enumerate}
\item Revise strong beliefs using (P1)-(P6),
\item Revise intentions using (P7)-(P12), possibly revising weak beliefs as well.
\end{enumerate}

Postulate (P7) states that the outcome of a revision should be coherent. Postulate (P8) states that the new intention $i$ take precedence over all other current intentions; if possible, it should be added, even if all current intentions have to be discarded. We can consider also not prioritized operators, which are not always successful. However, here we follow the standard approach in AGM theory change, which assumes that a check whether the belief base must be updated is done separately from the actual update.\footnote{Note that if we would drop postulate P8, then this would corresponding to dropping Item 2 of Definition~\ref{def:selection-function}.} Postulate (P9) and (P10) together state that if it is possible to simply add the intention, then this is the only change that is made. These two postulates are comparable to inclusion and vacuity of AGM. Postulate (P11) states that if we revise with the same $i$ but with a different belief, and we end up with the same belief in both cases, then we also end up with the same intentions. This postulate plays a crucial role in the interplay between beliefs and intentions, which we show in more detail in Example~\ref{expl:p11}. Finally, (P12) states that we do not discard intentions unnecessarily. This last postulate is a kind of maximality requirement, and is comparable to the \emph{parsimony requirement} introduced by~\cite{grant2010}.

We will show how revision works in our logic with various examples at the end of this section, after we have proved the representation theorem.

\subsection{Representation Theorem}
\label{sect:revision:representation}

In this subsection we present the main technical result of this paper. We characterize all revision schemes satisfying (P1)-(P12) in terms of minimal change with respect to an ordering among interpretations and a selection function accommodating new intentions while restoring coherence.

In the previous subsection we bounded various sets of formulas up to some time point $t$. We now do the same for models. We bound models up to $t$, which means that all the paths in the model are ``cut off'' at $t$. 

\begin{definition}[$t$-bounded model] 
\label{def:t-restrictedmodel}
Suppose some model $m=(T,\pi)$. 
\begin{itemize}
\item
A \emph{$t$-bounded path} $\restp{}$ is defined from a path $\pi$ in $T$ as $\restp{}=(\pi_0,\ldots,\pi_t)$. 
\item
A \emph{$t$-bounded model} $\restm{} = (\restt{},\restp{})$ is a pair where $\restt{}=\{\restp{}\mid \pi\in T\}$. 
\end{itemize}
We denote the set of all $t$-bounded models with $\restms{}$. 
\end{definition}

Recall we defined a set of models of strong beliefs \msbset{} as an \emph{msb set} (Definition~\ref{def:msbset}). A belief database $SB$ consists of a set of strong beliefs, and we showed in Proposition~\ref{prop:mod-sb-is-msbset} that the set of models of $SB$ is an msb set, i.e. $Mod(SB)\in\msbsets{}$, where $\msbsets{}$ is the set containing all msb sets.

In order to represent revision semantically, we define a $t$-bounded version of msb sets as well.

\begin{definition}[$t$-bounded msb set]
Given an msb set \msbset{} (definition~\ref{def:msbset}), the \emph{$t$-bounded msb set} contains all $t$-bounded models of \msbset{}, i.e. $$\msbsetrest = \{\restm \mid m\in \msbset\}.$$
\end{definition}

Given an intention database $I$, we define a selection function $\sel$ that tries to accommodate a new intention based on strong beliefs. The selection function specifies preferences on which intention an agent would like to keep in the presence of the new beliefs. 

\begin{definition}[Selection Function]
\label{def:selection-function}
Given an intention database $I$, a \emph{selection function} $\sel:\msbsets{}\times \ib \rightarrow \idb$ maps an msb set (Definition~\ref{def:msbset}) and an intention to an updated intention database---all bounded up to $t$--- such that if $\sel(\msbsetrest,\{i\})=I'$, then:
\begin{enumerate}
\item $(\msbsetrest,I')$ is coherent.
\item If $(\msbsetrest,\{i\})$ is coherent, then $i\in I'$.
\item If $(\msbsetrest,I\cup\{i\})$ is coherent, then $I\cup\{i\}\subseteq I'$.
\item $I'\subseteq I\cup\{i\}$.
\item For all $I''$ with $I'\subset I''\subseteq I\cup\{i\}$:$(\msbsetrest,I'')$ is not coherent.
\end{enumerate}
\end{definition}

The five conditions on the selection function are in direct correspondence with postulates (P7)-(P10), (P12) of the agent revision function $*_t$. Postulate (P11) doesn't have a corresponding condition in the definition above, but it is represented in the representation theorem below (Theorem~\ref{thm:singlestep}). In Condition 2 of the representation theorem, the selection function takes $Mod(\psi')$ as its first argument, which are the revised beliefs. This ensures the outcome of the intention revision process only depends on the new beliefs, the old intention database, and the incoming intention. In other words, it does not depend on the previous beliefs, or the belief that is used in revision. This is exactly what Postulate (P11) states as well.

\begin{remark}
We will show in Corollary~\ref{cor:strongbeliefformula} below that it is possible to represent each set of strong beliefs $SB$ (Definition~\ref{def:strbel}) by a formula $\psi$ such that $Cn(SB)=Cn(\psi)$. Using this corollary, we adapt the definition of a Katsuno and Mendelzon faithful assignment below.
\end{remark}

\cite{Katsuno1991} define a faithful assignment from a belief formula to a pre-order over models. Since we are also considering intentions, we extend this definition such that it also maps intentions databases to selection functions.

\begin{definition}[Faithful assignment]
\label{def:faithful-assignment}
A \emph{faithful assignment} is a function that assigns to each strong belief formula $\psi\in \sbel\rest{}$ a total pre-order $\lept$ over $\mods{}$ and to each intention database $I\in \mathbb{D}\rest{}$ a selection function $\sel$ and satisfies the following conditions:
\begin{enumerate}
\item If $m_1,m_2\in Mod(\psi)$, then $m_1\lept m_2$ and $m_2\lept m_1$.
\item If $m_1\in Mod(\psi)$ and $m_2\not\in Mod(\psi)$, then $m_1< m_2$.
\item If $\psi\equiv\phi$, then $\lept = \le_\phi^t$.
\item If $\restt=T_2\rest{}$, then $(T,\pi)\lept (T_2,\pi_2)$ and $(T_2,\pi_2)\lept (T,\pi)$.
\end{enumerate}
\end{definition}

Conditions 1 to 3 on the faithful assignment are the same as the conditions that Katsuno and Mendelzon put on a faithful assignment. Condition 4 ensures the two difficulties we pointed out in the beginning of this subsection are handled correctly:
\begin{itemize}
\item It ensures we do not distinguish between models in the total pre-order $\lept$ whose trees are the same up to time $t$. This is essentially what is represented in the revision function by bounding the all input of the revision function $*_t$ up to $t$. 
\item Moreover, $\lept$ does not distinguish between models obtained by selecting two different paths from the same tree. In other words, it ensures that msb sets (sets of models of a strong belief) remain in the same ordering. This corresponds to the fact that we are using strong belief formulas in the revision, which do not distinguish between different paths in the same tree as well.
\end{itemize}

We are now ready to state our main theorem.

\begin{theorem}[Representation Theorem]
\label{thm:singlestep}
A belief-intention revision operator $*_t$ satisfies postulates (P1)-(P12) iff there exists a faithful assignment that maps each $\psi$ to a total pre-order $\lept$ and each $I$ to a selection function $\sel$ such that if $(\psi,I)*_t(\varphi,i)=(\psi',I')$, then:
\begin{enumerate}
\item $Mod(\psi')=\min(Mod(\varphi),\lept)$
\item $I' = \sel(Mod(\psi'),i)$
\end{enumerate}
\end{theorem}

We will use the remainder of this subsection to prove the representation theorem above. We first show the number of $t$-bounded models is finite.

\begin{lemma} 
\label{lemma:finite-restricted-model}
For each $t\in\timeflow{},  \restms{}$ is finite. 
\end{lemma}

\begin{proof}
Suppose some $t\in\timeflow{}$. Since actions are deterministic and there are finitely many actions in our logic, each state has a finite number of successor states. Moreover, since there are finitely many propositions in our language, the number of possible valuations of the states is finite as well. Therefore, the number of models in $\restms{}$ is finite.
\end{proof}

The following lemma obtains a correspondence between semantic consequence of two models equivalent up to $t$. The proof is by induction on the depth of the formula.

\begin{lemma} 
\label{lemma:equivalent-entailment}
For each $\varphi\in \lang{}^{|t}$ and models $m_1,m_2\in\mods$, if $m_1^{|t}=m_2^{|t}$, then $m_1\models\varphi$ iff $m_2\models\varphi$.
\end{lemma}

Let $Ext(\msbsetrest)$ be the set of all possible extensions of a $t$-bounded msb set \msbsetrest{} to models, i.e. $$Ext(\msbsetrest) = \{m\in\mods{}\mid \restm{}\in \msbsetrest{}\}.$$ We next show that we can represent $\msbsetrest$ by a single strong belief formula using $Ext(\msbsetrest)$.

\begin{lemma}
Given a $t$-bounded msb set $\msbsetrest{}$, there exists a strong belief formula $form(\msbsetrest{})\in\mathbb{SB}$ such that $Mod(form(\msbsetrest))=Ext(\msbsetrest)$.
\end{lemma}

The following corollary shows we can represent a belief database consisting of strong beliefs up to some time $t$ with a single formula.

\begin{corollary}
\label{cor:strongbeliefformula}
Given a $t$-bounded set of strong beliefs $SB^{|t}$, there exists a strong belief formula $\psi\in\mathbb{SB}$ such that $SB^{|t}=\{\varphi\mid\psi\vdash\varphi\}$.
\end{corollary}

\subsection{Examples}
\label{sect:examples}

In this section we discuss various examples of revision of beliefs and intentions in our framework. We start with the example from the introduction, in which Bobby the household robot can only buy food and cleaning equipment if it robs a bank.

\begin{example}[Running example (robbing a bank)]
\label{expl:robbing}
Consider the following undesired situation. Suppose Bobby has a belief-intention database $(\psi, I)$ and that $I=\{(food, 0)\}$, i.e. Bobby intends to buy food at time 0. Now suppose Bobby would revise by the pair $(\top,(equip, 2))$: it would like to buy cleaning equipment at time 2. This is coherent (despite Bobby's belief that it does not have enough money for both) thanks to an action $rob$ of robbing a bank that it can perform at time 1. Suppose moreover that this is the only model where Bobby can perform both $(food, 0)$ and $(equip, 2)$. Then by postulate P8 we obtain that the resulting belief-intention database entails $do(rob)_1$, even if it would like to avoid robbing a bank by any means.

In other words, it seems that the weak beliefs of an agent may entail actions it did not intend to do, if those actions are the only means to carry out the intended actions. However, if Bobby would like to avoid robbing a bank by all means, then this should follow  explicitly in its strong belief database, i.e., for all $\ell$ (up to the considered  time  $t$) $$\psi\vdash \Box_0\neg do(rob)_\ell .$$
Given that this is a strong belief, the agent does not believe in any possible futures in which it rob a bank. A consequence of this is that the new intention $(equip, 2)$ will not be incorporated into the intention database, because the belief-intention database is not coherent after revision. If at some point later in time the agent would consider it possible to rob a bank, then it should revise its strong beliefs accordingly, but until that time the undesired action will not be weakly believed.
\end{example}

The above example shows that the agent can be coherent (it has the preconditions for all intended actions by postulate P8), but unaware of its future action to rob the bank (following from its weak beliefs). As shown in the example, this can be avoided by asserting this explicitly in the logic, however, due to belief revision this can change. If the agent really would never like to do this action, then this action should simply not be part of the available actions of the agent.

\begin{example}[Running example (adding an intention)]
\label{expl:addingintention}
Suppose a belief-intention database $(\psi,I)$ such that all models in $Mod(\psi)$ are the same as the partial model in Figure~\ref{fig:example_pal_model2} up to $t=2$ and suppose that $I=\{(food,0),(cook,1)\}$. That is, Bobby has the intention to buy food at time 0 and then to cook at time 1. Suppose now Bobby changes its intention to buy cleaning equipment at time 1. Formally: $$(\psi,I)*_1 (\top,(equip,1))=(\psi,I').$$  
First note $(\psi,I\cup\{(equip,1)\})$ is not coherent because no two intentions can occur at the same time moment. Moreover, since $(\psi,(equip,1))$ is coherent, from (P8) and (P9) we obtain $(equip,1)\in I'$. Furthermore, from (P10) we have that $I'\subseteq \{(food,0),(cook,1),(equip,1)\}$. Finally, $(\psi,\{(food,0),(equip,1)\})$ is not coherent either, since the agent does not believe the preconditions of buying food and buying equipment are true along a single path. Combining this gives $I'=\{(equip,1)\}$ as the only coherent outcome. Thus, Bobby no longer intends to buy food and to cook, but to buy cleaning equipment instead.

Note that, although the strong beliefs didn't change after revising with the new intention, the weak beliefs did change. For example, $post(food)_1\in WB(\psi,I)\setminus WB(\psi,I')$ and $post(equip)_2\in WB(\psi,I')\setminus WB(\psi,I)$.
\end{example}

The revision function $*_t$ takes a tuple $(\varphi,i)$ as input, and the postulates (P1)-(P7) ensure that revision of strong beliefs occurs prior to the revision of intentions. Therefore, it may seem plausible that revising with $(\varphi,i)$ is the same as first revising with $(\varphi,\epsilon)$ and then with $(\top,i)$. In other words, the following postulate seems to follow:

\begin{align*}
\text{If }&(\psi,I)*_t(\varphi,i)=(\psi',I')\\
\text{ and }&((\psi,I)*_t (\varphi,\epsilon))*_t (\top,i)=(\psi'',I''), \tag{P13*}\\
&\text{then }\psi'\equiv\psi''\text{ and }I'=I''.
\end{align*}

However, this property does not follow from (P1)-(P12), and we show in the following example that adding the postulate would in fact conflict with the maximality postulate (P12).

\begin{example}[Joint vs separate revision]
\label{expl:jointvsseparaterevision}
Suppose some belief-intention database $(\psi,I)$ with beliefs up to $t=2$ corresponding to the model on the left of Figure~\ref{fig:revision_example}. It is possible to go to the dentist ($dentist$) or to stay at work ($work$), and after that to go eating ($eating$) or go to the movies ($movies$). 

Before revision, the intentions are $I=\{(dentist,0),(eat,1)\}$ (left image of Figure~\ref{fig:revision_example}, intentions shown as bold lines). 

\begin{figure}[ht!]
\centering
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[level distance=2.5cm, 
	level 1/.style={sibling distance=2.5cm},
	level 2/.style={sibling distance=1.5cm},
	emph/.style={edge from parent/.style={ultra thick,draw}},
	norm/.style={edge from parent/.style={black,thin,draw}},
	grow'=right]
  \coordinate
    child{
      child{node{} edge from parent node[above]{$eat$}}
      child{node{} edge from parent node[below]{$movie$}}
      edge from parent node[above]{$work$}
    }
    child[emph]{
    child{node{} edge from parent node[above]{$eat$}}
      child[norm]{node{} edge from parent node[below]{$movie$}}
      edge from parent node[below]{$dentist$}
    }
  ;
\end{tikzpicture}
\end{minipage}
\hspace{1cm}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[level distance=2.5cm, 
	level 1/.style={sibling distance=2.5cm},
	level 2/.style={sibling distance=1.5cm},
	emph/.style={edge from parent/.style={ultra thick,draw}},
	red/.style={edge from parent/.style={ultra thick,draw=red,dashed}},
	norm/.style={edge from parent/.style={black,thin,draw}},
	invisible/.style={edge from parent/.style={white,thin,draw}},
	grow'=right]
  \coordinate
    child{
      child{node{} edge from parent node[above]{$eat$}}
      child{node{} edge from parent node[below]{$movie$}}
      edge from parent node[above]{$work$}
    }
    child{
    child[invisible]{node{} edge from parent node[above]{}}
      child{node{} edge from parent node[below]{$movie$}}
      edge from parent node[below]{$dentist$}
    }
  ;
\end{tikzpicture}
\end{minipage}
\caption{Left: Partial model of strong beliefs $\psi$ of agent $(\psi,I)$ with $I=\{(dentist,0),(eat,1)\}$ (bold lines). Right: Revised strong beliefs of agent after learning it is not possible to eat ($eat$) after the dentist ($dentist$).}
\label{fig:revision_example}
\end{figure}

Suppose now the beliefs are revised with the fact that it is not possible to go eating after going to the dentist ($\varphi$) and with the intention to go to the movie at time 1 ($i=(movie,1)$). The resulting strong beliefs after revising with $\varphi$ are shown on the right of Figure~\ref{fig:revision_example}.

Let us analyze two ways of revising this information:
\begin{itemize}
\item Suppose $(\psi,I)$ is revised with both the new belief and the new intention. That is, $$(\psi,I)*_2(\varphi,i)=(\psi',I').$$Both $(\psi',\{(dentist,0),(movie,1)\})$ and $(\psi',\{(movie,1)\})$ are coherent, so by the maximality postulate (P12), $I'=\{(dentist,0),(movie,1)\}$. Hence, the new intentions are to go to the dentist and then to go to the movie.
\item Suppose beliefs are revised prior to intentions. That is,
\begin{align*}
(\psi,I)*_2(\varphi,\epsilon)&=(\psi',\overline{I})\\
(\psi',\overline{I})*_2(\top,i)&=(\psi',\overline{I}').
\end{align*}
Now, since $(\psi',\{(dentist,0)\})$ and $(\psi',\{(eating,1)\})$ are both coherent, we either have $\overline{I}=\{(dentist,0)\}$ or $\overline{I}=\{(eating,1)\}$. Suppose that $\overline{I}=\{(eating,1)\}$. In that case, since $(\psi',\{(eating,1),(movie,1)\}$ is incoherent, we obtain $\overline{I}'=\{(movie,1)\}$ by the postulates (P8) and (P10).  
\end{itemize}

Thus, (P13*) doesn't hold. We see that revising separately allows a choice between the intention to go eating or to go to the dentist after revising beliefs. When choosing to go eating, the intention again has to be discarded because it is conflicting with the new intention to go to the movie. In joint revision, this is not the case since the choice between eating or the dentist can be made in light of the new incoming intention, and the maximal set can be chosen.
\end{example}

We use the next example to explain postulate P11.

\begin{example}
\label{expl:p11}
Suppose
\begin{align*}
(\psi,I)*_t(\varphi,i)&=(\psi',I')\\
(\psi_2,I)*_t(\varphi_2,i)&=(\psi',I_2'),
\end{align*}
then postulate P11 ensures $I'= I'_2$. In words, this means that whenever we revise an intention database $I$ by an intention $i$ and we obtain the same strong beliefs $\psi'$, then the new intention database should also be the same.

\begin{figure}[ht!]
\centering
\begin{tikzpicture}[level distance=2.5cm, 
	level 1/.style={sibling distance=2.5cm},
	level 2/.style={sibling distance=1.5cm},
	emph/.style={edge from parent/.style={ultra thick,draw}},
	red/.style={edge from parent/.style={ultra thick,draw=red,dashed}},
	norm/.style={edge from parent/.style={black,thin,draw}},
	invisible/.style={edge from parent/.style={white,thin,draw}},
	grow'=right]
  \coordinate
    child{
      child{
        child{node{} edge from parent node[above]{$nop$}}
        edge from parent node[above]{$spag$}
      }
      child{
        child{node{} edge from parent node[below]{$coffee$}}
        edge from parent node[below]{$nop$}
      }
      edge from parent node[above]{$beer$}
    }
    child{
      child{
          child{node{} edge from parent node[below]{$nop$}}
          child{node{} edge from parent node[below]{$coffee$}}
          edge from parent node[below]{$spag$}
      }
      edge from parent node[above]{$nop$}
    }
  ;
\end{tikzpicture}
\caption{Tree representing Bobby's strong beliefs $\psi'$ up to time $t=2$ (Example~\ref{expl:p11})}
\label{fig:revision_example2}
\end{figure}

Suppose for instance our household robot Bobby has the intention database $I=\{(beer,0),(spag,1)\}$, i.e. it intends to buy beer at time 0 and to buy spaghetti at time 1. Suppose now Bobby learns it only has sufficient money to either buy beer and spaghetti, or beer and coffee. Bobby's beliefs $\psi'$ are represented up to time 2 by the tree in Figure~\ref{fig:revision_example2}. If Bobby also adopts the intention to buy coffee at time 3, i.e. $i=(coffee,3)$, then it should either drop $(beer,0)$ or $(spag,1)$ in order to incorporate $i$. Postulate P11 ensures that this choice is independent of its beliefs prior to revising them. 
\end{example}

